DALL-M: Context-Aware Clinical Data Augmentation with LLMs

X-ray images are vital in medical diagnostics, but their effectiveness is limited without clinical context. Radiologists often find chest X-rays insufficient for diagnosing underlying diseases, necessitating the integration of structured clinical features with radiology reports. To address this, we introduce DALL-M, a novel framework that enhances clinical datasets by generating contextual synthetic data. DALL-M augments structured patient data, including vital signs (e.g., heart rate, oxygen saturation), radiology findings (e.g., lesion presence), and demographic factors. It integrates this tabular data with contextual knowledge extracted from radiology reports and domain-specific resources (e.g., Radiopaedia, Wikipedia), ensuring clinical consistency and reliability. DALL-M follows a three-phase process: (i) clinical context storage, (ii) expert query generation, and (iii) context-aware feature augmentation. Using large language models (LLMs), it generates both contextual synthetic values for existing clinical features and entirely new, clinically relevant features. Applied to 799 cases from the MIMIC-IV dataset, DALL-M expanded the original 9 clinical features to 91. Empirical validation with machine learning models (including Decision Trees, Random Forests, XGBoost, and TabNET) demonstrated a 16.5% improvement in F1 score and a 25% increase in Precision and Recall. DALL-M bridges an important gap in clinical data augmentation by preserving data integrity while enhancing predictive modeling in healthcare. Our results show that integrating LLM-generated synthetic features significantly improves model performance, making DALL-M a scalable and practical approach for AI-driven medical diagnostics.

==> tab_lit_rev_back.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Approach} &
  \textbf{Key Focus} &
  \textbf{Limitations} &
  \textbf{Role of DALL-M} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ChiMed-GPT \citep{tian2023chimed}, \\ MedicalGPT \citep{Xu2023}, \\ HuatuoGPT-II \citep{chen2023huatuogpt}, \\ ChatMed \citep{zhu2023chatmed}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Adapt general-domain LLMs \\ for clinical tasks\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Primarily focused on text-based reasoning \\ (e.g., question answer tasks)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Leverages LLMs in a novel way to enrich \\ \textit{tabular} data with new features and \\ synthetic values\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Harness large-scale medical \\ text corpora\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Less attention to generating entirely new \\ clinical features\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Goes beyond question-answering by creating \\ entirely new features relevant to specific \\ radiology contexts\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Provide domain-specific \\ responses (e.g., diagnoses)\end{tabular} &
  Limited exploration of tabular data &
  Focuses on text and tabular data \\ \hline
\multirow{2}{*}{ClinicalT5 \citep{lu2022clinicalt5}} &
  \begin{tabular}[c]{@{}l@{}}Fine-tuned T5 for clinical text tasks\\  (e.g., summarizing patient records)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Focus on generating or refining text-based \\ outputs, not specialized in augmenting \\ structured (tabular) clinical data with new \\ features\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}DALL-M introduces a three-phase pipeline \\ that leverages multiple data sources to create \\ augmented tabular data\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Shows improved performance in \\ typical NLP tasks such as entity \\ recognition, summarization\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Does not explore advanced context \\ integration (e.g., from multiple sources \\ like Radiopaedia, Wikipedia)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Adds clinically relevant features rather than \\ just refining text\end{tabular} \\ \hline
\multirow{2}{*}{ClinicalGPT \citep{wang2023clinicalgpt}} &
  \begin{tabular}[c]{@{}l@{}}Integrates various info sources \\ (medical records, domain knowledge, \\ dialogues)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Emphasis on multi-round consultations \\ and EHR text retrieval\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}DALL-M not only consolidates domain \\ knowledge from multiple sources but also \\ generates new, context-aware \\ \emph{tabular} features\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Enables context-rich responses in \\ interactive clinical settings\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}No explicit mechanism for structured \\ tabular feature augmentation or generation \\ of new features\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Uses a retrieval-augmented pipeline to \\ ensure alignment of new features with \\ established clinical knowledge\end{tabular} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}BioGPT \citep{Luo2022} \\ PubMedBERT \citep{gu2021domain} \\ GatorTron \citep{yang2022large}\end{tabular}} &
  Domain-trained LLMs &
  \begin{tabular}[c]{@{}l@{}}Specialized for textual data (biomedical \\ corpora, EHR text) with minimal focus on \\ synthetic feature generation in numerical \\ or tabular formats\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}DALL-M embeds new numeric or categorical \\ features into existing tabular records, \\ preserving consistency and context\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Enhanced accuracy in medical text \\ classification, knowledge extraction, etc\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Do not address missing data or new feature \\ creation in a robust data-augmentation setting\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Addresses missing data scenarios and introduces \\ novel features (e.g., additional vital stats, \\ symptom descriptors)\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Med-PaLM \citep{singhal2023large}\\ MedAlpaca \citep{han2023medalpaca}\\ LLaVA-Med \citep{li2024llava}\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Employ large-scale domain adaptation \\ of general LLMs\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Focus primarily on question-answer or generative\\  tasks (report summarization, explanations)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}DALL-M explicitly tackles the augmentation \\ of \emph{tabular} clinical data with entirely new \\ features (not just text or imaging commentary)\end{tabular} \\ \cline{2-4} 
 &
  Incorporate specialized medical data &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Limited exploration of how to augment \emph{structured,}\\ \emph{tabular} clinical data with newly \\ inferred features\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uses multi-modal and multi-source knowledge \\ (X-rays + textual reports + Radiopaedia + Wikipedia) \\ for robust feature generation\end{tabular}} \\ \cline{2-2}
 &
  \begin{tabular}[c]{@{}l@{}}Provide multi-modal understanding \\ (images + text)\end{tabular} &
   &
   \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}TDA \\ (e.g. Noise Injections, \\ Data Permutations)\end{tabular}} &
  Simple to implement for numeric data &
  \begin{tabular}[c]{@{}l@{}}Often breaks clinical consistency (random \\ noise can create medically implausible \\ combinations)\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}DALL-M preserves clinical logic by integrating \\ domain knowledge from multiple sources and \\ structured expert queries\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Can increase dataset size quickly \\ for ML model training\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Does not leverage domain knowledge to ensure \\ realism or generate completely new features\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}-Ensures newly generated or augmented features \\ remain medically plausible\end{tabular} \\ \hline
\multirow{4}{*}{\textbf{DALL-M (Our Study)}} &
  \begin{tabular}[c]{@{}l@{}}Generates synthetic, context-relevant \\ numeric values for missing data\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Requires advanced retrieval-augmented methods \\ and curated knowledge sources\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Fills the gap of systematically augmenting tabular \\ data with \emph{both} realistic values for existing \\ columns and \emph{entirely new} clinically relevant \\ features\end{tabular} \\ \cline{2-4} 
 &
  \begin{tabular}[c]{@{}l@{}}Creates entirely new features based on \\ domain knowledge and retrieval\\ augmented LLM queries\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Dependent on LLM frameworks (e.g., GPT-4) \\ for best performance, which can be computationally \\ expensive\end{tabular} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Provides robust, context-aware augmentation \\ that improves downstream ML performance and \\ addresses missing data issues\end{tabular}} \\ \cline{2-3}
 &
  \begin{tabular}[c]{@{}l@{}}Integrates multiple data sources \\ (e.g., Radiopaedia, Wikipedia) and \\ expert inputs\end{tabular} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ethical and privacy guidelines for synthetic data \\ must be carefully observed\end{tabular}} &
   \\ \cline{2-2}
 &
  \begin{tabular}[c]{@{}l@{}}Demonstrates efficacy across multiple\\ ML models (e.g., XGBoost, TabNet)\end{tabular} &
   &
   \\ \hline
\end{tabular}
}
\caption{Summary of LLM-Based Approaches for Data Augmentation.}
\label{tab:lit_rev}
\end{table}
